Network Generation with Differential Privacy

We consider the problem of generating private synthetic versions of real-world graphs containing private information while maintaining the utility of generated graphs. Differential privacy is a gold standard for data privacy, and the introduction of the differentially private stochastic gradient descent (DP-SGD) algorithm has facilitated the training of private neural models in a number of domains. Recent advances in graph generation via deep generative networks have produced several high performing models. We evaluate and compare state-of-the-art models including adjacency matrix based models and edge based models, and show a practical implementation that favours the edge-list approach utilizing the Gaussian noise mechanism when evaluated on commonly used graph datasets. Based on our findings, we propose a generative model that can reproduce the properties of real-world networks while maintaining edge-differential privacy. The proposed model is based on a stochastic neural network that generates discrete edge-list samples and is trained using the Wasserstein GAN objective with the DP-SGD optimizer. Being the first approach to combine these beneficial properties, our model contributes to further research on graph data privacy.

==> review.tex <==
% \section{Background of Network Generation}
% The use of generative models to create entire graph structures has drawn substantial attention from the research community in the past few years. In recent work \cite{tavakoli2017learning}, the author applies GANs to graph data by trying to create adjacency matrices of social networks directly. In this model, the generator tries to generate the flattened adjacency matrix. The discriminator is provided with generated adjacency matrix along with 10,000 permutations of the original adjacency matrix with randomly swapped node indexes. Their model successfully captures several useful aspects of the graphs like node degrees and network diameter. Another work \cite{fan2019labeled} also uses adjacency matrices to generate labeled nodes with the advantages of graph neural network \cite{scarselli2008graph}. Experiment results show that this model can generate diverse labeled graphs that match the training data structural characteristics. Though these models can generate graphs that match the training adjacency matrix's structural characteristics, they require computations and memory quadratic in the number of nodes. Such quadratic complexity is infeasible in practice for big graphs, allowing them to process only small graphs. Another direction is using deep learning methods for graph data in the context of node embeddings. The main idea behind these approaches is modeling the probabilities of each edge’s existence by a neural network \cite{perozzi2014deepwalk}. The recently proposed GraphGAN \cite{wang2018graphgan} is an instance of such prescribed edge-level probabilistic models, using the GAN objective instead of the traditional cross-entropy to optimize the probabilities of each individual edge’s existence. Deep embedding based methods achieve state-of-the-art scores in tasks like link prediction and node classification. Nevertheless, such approaches for generating entire graphs produce samples that don’t preserve any of the patterns inherent to real-world networks. 

% In contrast, NetGAN \cite{bojchevski2018netgan} operates random walks on the input graphs\cite{lovasz1993random}, and the generator tries to mimic these walk sequences with LSTM \cite{hochreiter1997long} architecture. After trained, the generator can crate a batch of walk sequences and consists a adjacency matrix with these walks. NetGAN considers only the non-zero entries of the adjacency matrix efficiently exploiting the sparsity of real-world graphs, and is readily applicable to graphs with thousands of nodes.

% \subsection{Differential privacy and Deep Learning}
% Differential privacy is considered as one of the strongest privacy definitions, which addresses the paradox of learning nothing about an individual while learning useful information about a population \cite{dwork2014algorithmic}. It gives a quantitative mathematical definition to measure the level of privacy that can be achieved by an algorithm or function. In the context of data synthesis, it is not a measure that applies to the new data but to the models that create this synthetic data. Formal definitions and properties of differential privacy are introduced in this section.   

% \textbf{Adjacent Database.} Before talking about differential privacy, we need to first define a application-specific concept of adjacent databases - two datasets are adjacent if they differ in a single entry, that is, if one image-label pair is present in one set and absent in the other in an image dataset. 

% \textbf{Differential Privacy Definitions} A randomized algorithm $M$ gives $(\epsilon, \delta)$-differential privacy if, for any adjacent databases $d$ and $d'$, differing on at most one element and all $S \in Range(M)$.

% \begin{equation}
%     Pr[ M(d) \in S] \leq exp(\epsilon) \times Pr[M(d') \in S] + \delta 
% \end{equation}\label{eq:mechanism}

% To enable differential privacy for a given deterministic function $f$, we can inject random noise into $f$'s output, where the noise amount is determined by $f$'s sensitivity, defined as

% \begin{equation}
% \Delta f = max_{d, d'}\|f(d) - f(d')\|
% \end{equation}\label{eq:sensitivity}
% where $\Delta f$ is the maximum influence of a single data point on the output of $f$. Given the above definition, a common choice is to apply the Gaussian mechanism \cite{dwork2014algorithmic} to $f$'s output, where $N(0, (\Delta f)^2 \sigma^2 I)$ is a Gaussian distribution with zero mean and standard deviation $\Delta f \sigma$.:
% \begin{equation}
% M(d) = f(d) + N(0, (\Delta f)^2 \sigma^2),
% \end{equation}\label{eq:Gaussian}

% The following theorems, which are proved in work \cite{dwork2014algorithmic},  are two useful properties that allow us to integrate differential privacy with machine learning algorithms.

% \textbf{Post Processing Theorem.} Given the above $(\epsilon, \delta)$-DP algorithm $M$, and let $f: R \rightarrow \hat{R}$ be any randomized function. Then, $f \cdot M : \mathbb{N}^{|X|} \rightarrow \hat{R}$ is also $(\epsilon, \delta)$-DP \cite{dwork2014algorithmic}.

% % Keeping track of the accumulated privacy loss in the course of execution of a composite mechanism, and enforcing the applicable privacy policy, can be performed by the privacy accountant..,.
% \textbf{Composition Theorem.} Differential privacy for repeated applications of additive-noise mechanisms follows the basic composition theorem \cite{dwork2014algorithmic}, or advanced composition theorems and their refinements\cite{mironov2017renyi}. In work \cite{abadi2016deep}, the author has applied differential privacy mechanisms in the training of deep learning models by adding Gaussian noise to the gradients. This method requires the addition of random noise to the computed gradients to obfuscate the influence that an input data can have on the final model. They developed NoisySGD and Moment accountant, which keeps track of a bound on privacy loss moments during the training procedure of a deep neural network.
% \begin{figure}[h]
% \centering
% \includegraphics[width=0.9\linewidth]{assets/dp-gan.png}
% \caption{The general process of training a differentially private GAN. The noise is added on the gradients of the discriminator.}
% \label{dp_gan_architecture}
% \end{figure}

% DPGAN \cite{xie2018differentially} developed a method to train GANs in a differentially private manner. This model relies on the Post-Processing Theorem to change the problem from learning a differentially private generator to the task of learning a differentially private discriminator. Similar with work \cite{abadi2016deep}, the key idea is that noise is added to the gradients, but in DPGAN, the noise is only added on the gradients of discriminator during training. Figure \ref{dp_gan_architecture} shows the general process of training a differential private GAN.

% PATEGAN \cite{jordon2018pate} is another way using modifies the Private Aggregation of Teacher Ensembles (PATE) framework \cite{papernot2016semi} and applies it to GANs. It can generate synthetic multi-variate tabular data without compromising the privacy of training data. The PATE framework provides a differentially private mechanism for classification by training multiple teacher models on disjoint partitions of the data. To classify a new sample, each teacher’s output is evaluated on the sample, and then all outputs are noisily aggregated. In PATEGAN, a set of \textsc{teacher} discriminators are trained separately with disjoint partitions of the training set. A \textsc{student} discriminator is trained with generated samples, labelled by the noisy aggregated labels from all teachers. The generator is trained to minimize the loss with respect to the student discriminator. In this process, the student discriminator does not access the training set and keep differentially private. Benefit from the Post Processing Theorem, the generator trained against the student discriminator is thus differentially private.




